Distributed Primal-Dual Interior Point Framework for Analyzing Infeasible Combined Transmission and Distribution Grid Networks

The proliferation of distributed energy resources has heightened the interactions between transmission and distribution (T&D) systems, necessitating novel analyses for the reliable operation and planning of interconnected T&D networks. A critical gap is an analysis approach that identifies and localizes the weak spots in the combined T\&D networks, providing valuable information to system planners and operators. The research goal is to efficiently model and simulate infeasible (i.e. unsolvable in general settings) combined positive sequence transmission and three-phase distribution networks with a unified solution algorithm. We model the combined T&D network with the equivalent circuit formulation. To solve the overall T&D network, we build a Gauss-Jacobi-Newton (GJN) based distributed primal dual interior point optimization algorithm capable of isolating weak nodes. We validate the approach on large combined T&D networks with 70k+ T and 15k+ D nodes and demonstrate performance improvement over the alternating direction method of multipliers (ADMM) method.

==> Sections/extras.tex <==
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\linewidth]{images/VEC_infeasi_L2.png}
    \caption{A graph representation of the South-Hero substation with a heatmap showing the highest infeasibility current magnitude at each node, based on the L2 norm formulation.}
    \label{fig:subfig1}
\end{figure}
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\linewidth]{images/VEC_infeasi_L1.png}
    \caption{A graph representation of the South-Hero substation with a heatmap showing the highest infeasibility current magnitude at each node, based on the L1 norm formulation.}
    \label{fig:subfig2}
\end{figure}
